Computing Real Numbers with Large-Population Protocols Having a Continuum of Equilibria

Bournez, Fraigniaud, and Koegler defined a number in [0,1] as computable by their Large-Population Protocol (LPP) model, if the proportion of agents in a set of marked states converges to said number over time as the population grows to infinity. The notion, however, restricts the ordinary differential equations (ODEs) associated with an LPP to have only finitely many equilibria. This restriction places an intrinsic limitation on the model. As a result, a number is computable by an LPP if and only if it is algebraic, namely, not a single transcendental number can be computed under this notion. In this paper, we lift the finitary requirement on equilibria. That is, we consider systems with a continuum of equilibria. We show that essentially all numbers in [0,1] that are computable by bounded general-purpose analog computers (GPACs) or chemical reaction networks (CRNs) can also be computed by LPPs under this new definition. This implies a rich series of numbers (e.g., the reciprocal of Euler's constant, $\pi/4$, Euler's $\gamma$, Catalan's constant, and Dottie number) are all computable by LPPs. Our proof is constructive: We develop an algorithm that transfers bounded GPACs/CRNs into LPPs. Our algorithm also fixes a gap in Bournez et al.'s construction of LPPs designed to compute any arbitrary algebraic number in [0,1].

==> rachels_sections/detailed_termolecular_construction.tex <==
%!TEX root = ../main.tex
Given an algebraic number $\nu\in[0,1]$, its minimal polynomial can be written as $\sum_{i=0}^\delta a_ix^i$ where $\delta$ is the polynomial’s degree.  Let $f(x)=\text{sgn}(a_0)\cdot \text{minpoly}(\nu)$. In addition, let $p(x)$ be the sum of positiver terms and $-x\cdot q(x)$ be the sum of negative terms in $f(x)$. Then we can write $f(x)=p(x)-x\cdot q(x)$.

In the first step, we obtain a system of differential equations in the variable $x$. Define the derivative of $x$ as $x ' = p(x)-x\cdot q(x)$. Then, find the derivatives of $x^2 , x^3, \dots, x^\delta$ using the chain rule and the substitution of $x'$.  For $i=2,\dots,\delta$, we have
%
\begin{align*}(x^i)' &= i x^{i-1} \cdot x' \\ &= ix^{i-1}\left[ p(x)-x\cdot q(x)\right] \\ &= ix^{i-1} \cdot p(x)- ix^i \cdot  q(x).\end{align*}
%

For the second step, we introduce and perform a change of variables. Introduce new variables such that $x_i:= x^i$ for $i=1,\dots,\delta$. Performing the change of variables yields,
%
\[\begin{cases}
x_1' &= p(x)-x_1\cdot q(x) \\
x_i' &= ix_{i-1} \cdot p(x) - ix_i \cdot q(x)  \quad\quad i=2,\dots,\delta.
\end{cases}\]
%
Note that $x_i$ is a factor of every negative term in  $x_i'$ for $i=1,\dots,\delta$.
%

In the third step, we introduce a variable $x_0$ for conservation of the system. Multiply each differential equation from the second step by $x_0$. Then add the differential equation $x_0'=-\sum_{i=1}^\delta x_i'$ to the system. For any terms with degree less than three, multiply the term by $1=\sum_{i=0}^\delta x_i$. As a result, we have the conserved termolecular system,
%
\[\begin{cases} x_1' &= x_0\left[p(x)-x_1\cdot q(x) \right]\\ x_i' &= x_0\left[ix_{i-1} \cdot p(x) - ix_i \cdot q(x)\right]  \quad i=2,\dots,\delta \\ x_0'&= -\sum\limits_{i=1}^\delta x_i'\end{cases}\]
%
whose initial configuration is defined as $x_0(0)=1$ and $x_i(0)=0$ for $i=1,\dots,\delta$.


==> rachels_sections/final_attempt.tex <==
%!TEX root = ../main.tex
\begin{proof}
Let $\mathcal{P}_x$ be a protocol described by state set $\bx =(x_0, x_1,\dots,x_n)$ and the differential system,
%
\[
\bx' =
\begin{cases} x_i'&=[p(x)-x_iq(x)]\cdot x_0, \quad \forall i\in \{1,\dots,n\}\\ x_0'&= -\sum\limits_{i=1}^n x_i'\end{cases}
\]
%
where $p(x)\in\pospoly$ is a quadratic form, $q(x)\in\pospoly$ is a linear form, and $x_1$ computes some number $\alpha$. Assume $\mathcal{P}_x$ is initialized such that $x_0(0)=1$ and $0$  otherwise.

We construct a population protocol based on the observation,
%
\[
\sum_{i=0} ^n x_i  \cdot \sum_{j=0} ^n x_j =1\cdot 1 =1.
\]
%
First, we define the new state set, $\mathbf{z}$.
Introduce new variables $z_{i,j}=x_ix_j$  for all $(x_i,x_j)\in \bx\times \bx$. To compute $\alpha$, define the marked states as $M_\mathbf{z}=\{z_{1,i} \mid i=1,\dots, n \}$.
%

Second, we define the initial configuration $\mathbf{z}(0)$. Let $z_{i,j}(0)=x_i(0)\cdot x_j(0)$ for all $(x_i, x_j)\in \bx \times \bx$.

Third, we define the new system of differential equations, $\mathbf{z'}$. For all $ x_i, x_j \in \bx$ we have $z_{i,j}'=(x_ix_j)'=x_i'x_j + x_ix_j'$, where $x_i', x_j'\in \bx'$. Recall that the differential equations of $\bx'$ are cubic forms. Therefore, $x_i'x_j + x_ix_j'$ is a quartic form. It follows from the change of variables from $\bx$ to $\mathbf{z}$ that $z_{i,j}'$ is a quadratic form.
%
For each $z_{i,j}\in \mathbf{z}$, we show that $z_{i,j}'$ satisfies the following two conditions: $(i)$ $z_{i,j}$ is a factor of every negative term in $z_{i,j}'$, and $(ii)$ there is no positive $z_{i,j}^2$  in $z_{i,j}'$. \todo{Keep or replace with conditions lemma?} There are three nontrivial cases.

%%% CASE 1
Case 1: Given $z_{i,j} = x_ix_j$ such that $i\neq 0$ and $j\neq 0$, we have
%
\begin{align*}
 z_{i,j}' &= x_i'x_j+x_ix_j'
 \\
 &= [p(x) - x_i q(x) ] \cdot x_0 \cdot x_j + x_i\cdot [p(x) - x_j q(x) ] \cdot x_0
 \\
 &=[{x_0 x_j p(x)} + {x_0 x_i p(x)} ]- 2 x_i x_j x_0 q(x).
\end{align*}
%
Since $x_i x_j$  can be factored out of every negative term, condition $(i)$ is met.
Since $x_0$ is a factor of every positive term, condition $(ii)$ is satisfied when $i\neq 0$ and $j\neq 0$.
%%% CASE 2
Case 2: Given $z_{0,j}$ such that $j\neq 0$, we have $z_{0,j}'
= x_0' x_j + x_0 x_j'$.
%
Note that
%
\begin{align*}z_{0,j}'&= x_0' x_j + x_0 x_j'
  \\
  &=\sum\limits_{i=1}^n  [q(x)x_i - p(x)]\cdot x_0 \cdot x_j + x_0\cdot [p(x)-x_j q(x)]\cdot x_0
  \\
  &= \left[\sum\limits_{i=1}^n  q(x)x_0x_jx_i - \sum\limits_{i=1}^np(x)x_0 x_j \right]+\left[ p(x)x_0^2-x_j q(x)x_0^2  \right]
  \\
  &= \left[p(x)x_0^2 + \sum\limits_{i=1}^n  q(x)x_0x_jx_i
 \right]-\left[ x_j q(x)x_0^2 + \sum\limits_{i=1}^np(x)x_0 x_j   \right].
\end{align*}
%
Since $x_0x_j$ can be factored from every negative term, condition $(i)$ is satisfied.
Suppose a positive term in $z'_{0,j}$ has the monomial $(x_0x_j)^2$. By carefully choosing the change of variable (i.e., choose $z_{j,j}z_{0,0}$, not $z_{0,j}^2$), we satisfy condition $(ii)$. If there is no positive term in $z'_{0,j}$ with the monomial $(x_0x_j)^2$, then condition $(ii)$ is met.


%%% CASE 3

Case 3: Given $z_{0,0}$ , we have
%
\begin{align*}
  z_{0,0}' &= 2x_0 \cdot x_0'
  \\
  &= 2x_0 \cdot\sum\limits_{i=1}^ n [q(x)x_i-p(x)]\cdot x_0
  \\
  &= {\sum\limits_{i=1}^ n 2x_0^2 q(x)x_i} - {\sum\limits_{i=1}^ n 2x_0^2 p(x)}.
\end{align*}
%
Since $x_0^2$ can be factored from every negative term, condition $(i)$ is satisfied.
Since   $i=1,\dots,n$ , it follows that $x_i\neq x_0$. Thus, condition $(ii)$ is satisfied.
%

In summary, we have defined the states $\mathbf{z}$, marked states $M_\mathbf{z}$, initial configuration $\mathbf{z}(0)$, and differential system $\mathbf{z'}$. Furthermore, for each $z_{i,j}'\in \mathbf{z'}$ we have established: each $z_{i,j}'$ is a quadratic form, $z_{i,j}'$ can be written to avoid a positive $z_{i,j}^2$ in $z_{i,j}'$, and the existence of $z_{i,j}$ in every negative term of $z_{i,j}'$. Hence, we have a population protocol $\mathcal{P}_z$ that computes $\alpha$.

\todo{show convervation carries from x to z}

\end{proof}


==> rachels_sections/termolecular.tex <==
We claim that there is a termolecular protocol $\mathcal{P}_3$ to compute any algebraic number $\nu\in[0,1]$, provided $\nu$ is the first positive root of its minimal polynomial. If $\text{minpoly}(\nu)=\sum_{i=1}^\delta a_i x^i$, define $f(x)=\text{sgn}(a_0)\cdot \text{minpoly}(\nu)$. Furthermore, define new variables $x_i:=x^i$ for $i=1,\dots, \delta$. The protocol is described by the system of differential equations,
%
  \[\begin{cases}
  x_1' &=x_0 \left[p(x)-x_1 q(x)\right] \\
  x_i' &= x_0 \left[ ix_{i-1} p(x) - ix_i q(x)\right] \quad \text{for } i=2,\dots,\delta   \\
  x_0' &= -\sum\limits_{i=1}^\delta x_i'
  \end{cases},\]
%
where:
  \begin{itemize}
    \item $\delta$ is the degree of $f(x)$,
    \item $p(x)$ is the sum of positive terms in $f(x)$, and
    \item $- x q(x)$ is the sum of negative terms in $f(x)$.
  \end{itemize}
%
Initialize the system such that $x_0(0)=1$ and $x_i(0)=0$ for $i=1,\dots,\delta$.

%TODO add in lambda trick information?

